Real-time Contact State Estimation in Shape Control of Deformable Linear Objects under Small Environmental Constraints

Controlling the shape of deformable linear objects using robots and constraints provided by environmental fixtures has diverse industrial applications. In order to establish robust contacts with these fixtures, accurate estimation of the contact state is essential for preventing and rectifying potential anomalies. However, this task is challenging due to the small sizes of fixtures, the requirement for real-time performances, and the infinite degrees of freedom of the deformable linear objects. In this paper, we propose a real-time approach for estimating both contact establishment and subsequent changes by leveraging the dependency between the applied and detected contact force on the deformable linear objects. We seamlessly integrate this method into the robot control loop and achieve an adaptive shape control framework which avoids, detects and corrects anomalies automatically. Real-world experiments validate the robustness and effectiveness of our contact estimation approach across various scenarios, significantly increasing the success rate of shape control processes.

==> sections/sec4_dynamics.tex <==
\section{Contact Dynamics}
In this section, we study the force interaction between the grasped DLO and the clip fixture during the insertion stage. 
Initially, the DLO establishes direct contact with the clip.
Subsequently, each robot applies a stretching force and a pushing force on the respective ends of the DLO, forcing it to be fixed into the clip. 
Throughout this process, the clip remains anchored to the ground, maintaining a consistent pose.

\begin{figure}[t]
    \centering
    \begin{tikzpicture}
    \node[inner sep=0pt] (russell) at (0,0)
    {\includegraphics[width=0.48\textwidth]{figures/foce_trans.png}};
    \node at (-0.3,-0.1) {(5)};
    \node at (1.35,-0.1) {(10)};
    \node at (3.8,-0.1) {(11)};
    \end{tikzpicture}
    \caption{Transmission of force.}
    \label{fig: force_trans}
    % \vspace{-1.7em} 
\end{figure}

Should a robot apply a force $\mathbf{f}$ onto a \textit{rigid} object $A$, which is in contact with another \textit{rigid} object $B$ securely affixed to the ground, the underlying dynamics can be summarized as $\mathbf{f^{ff}} = \mathbf{a} \cdot m_A  + \mathbf{f_c} \textbf{,}$ where $\mathbf{a}$ represents acceleration, $m_A$ represents the mass of object $A$, and $\mathbf{f_c}$ represents the contact force. 
In essence, these dynamics can be conceptualized as a system that takes $\mathbf{f^{ff}}$ as input and generates outputs in the form of $\mathbf{a}$ and $\mathbf{f_c}$. 
The contact dynamics could be then revealed by analysis of interrelationship between input and output.

We endeavor to apply a similar modeling approach to analyze the contact phenomena in the clip fixing process which can be considered as a system which takes feedforward force as input, and outputs detected force and movement as output.
However, due to the deformations exhibited by both the DLO and the clip, $\mathbf{f_c}$ does not exhibit a direct correspondence with $\mathbf{f^{ff}}$, but rather undergoes a series of transmission, as depicted in Fig~\ref{fig: force_trans}.
To figure out the transmission specifically,  we further analyze the intermediate force on each section of the DLO.

% We would like to analyze the contact in the clip fixing process using a similar model. 
% However, due to the deformation of the DLO and the clip, $\mathbf{f_c}$ is not in direct relationship with $\mathbf{f^{ff}}$, but experiences a series of transmission, as shown in Fig.
% In this section, We will look into these intermediate forces one by one.

\subsection{Overall Force Interaction}
\begin{figure}[t]
    \centering
    \begin{tikzpicture}
    \node[inner sep=0pt] (russell) at (0,0)
    {\includegraphics[width=0.48\textwidth]{figures/cable_dynamics.png}};
    \node at (-0.25,-0.6) {(a)};
    \node at (-1.8,-3.6) {(b)};
    \node at (2.5,-3.6) {(c)};
    \end{tikzpicture}
    \caption{Cable Dynamics in Contact with the Clip. (a) DLO dynamics with a force applied to the center. (b) Clip dynamics with force pushing the object inward. Note that we omitted the forces whose component in $Y$ direction is zero.}
    \label{fig: cable_dynamics}
    % \vspace{-1.7em} 
\end{figure}

The cable can be modeled as a non-elastic deformable linear object (DLO).
Without loss of generality, we assume that this DLO has uniformly distributed stiffness along $X$ axis. % We study specifically the dynamics of the grasped DLO as well as the clip at the insertion stage, which involves the most force interactions.
As is shown in Fig~\ref{fig: cable_dynamics}(a), contact with the clip fixture leads to the deformation of the grasped segment of DLO.
Since the DLO is stretched beforehand to remain tension, we assume there is no observable deformation along the DLO (stretching or press) during the insertion stage.
% The magnitude of the tension $\mathbf{f_s}$ can be thus formulated as a function of angle $\theta$
% \begin{equation} \label{equ: ff2fs}
%     ||\mathbf{f_s}(\theta(t))|| =  ||\mathbf{f^{ff}_{push}}|| \cdot \cos(\theta(t)) + ||\mathbf{f^{ff}_{stretch}}|| \cdot \sin(\theta(t))\textbf{.}
% \end{equation}
Taking all the external forces applied on the grasped DLO into account, the dynamics of the DLO can be described as
\begin{equation}
    m \cdot {\mathbf{a}}(t) = \mathbf{f^{ff}_{push}} - \mathbf{f_{c}}(t)\textbf{,}
\end{equation}
where $\mathbf{f_{c}}$ is the contact force applied on the DLO by the clip.

\subsection{Sectional Force Interaction}
Dependent on whether it is in contact with the fixture, the grasped DLO can be divided into three sections $\{s_i\}, i \in \{1,2,3\}$, each with length $l_i$  and mass $m_i$.
As each end of the grasped DLO is stretched by each robot with a symmetric force, we assume that there is no sliding in $X$ axis and the division remains constant as long as the contact is maintained (before inserted-in).

$s_2$ is in the central part of the DLO and is in direct touch with the clip.
As $s_2$ holds a solid contact with the fixture, we consider it possesses high stiffness and its own deformation can be ignored.
The interaction between the clip and the DLO can be analyzed based on the clip dynamics described in Section~\ref{subsec: clip_dynamics}.
Considering the forces on $s_2$, the actuation force $\mathbf{f}$ in this case is a component of the tension in $Y$ direction:
\begin{equation} \label{equ: s2_time_variant}
     ||\mathbf{f}(\theta(t))|| = 2||\mathbf{f_s}(\theta(t))|| \cdot sin(\theta(t))\textbf{,}
\end{equation}
which varies with time as $\theta(t)$ varies.

% $s_1$ and $s_3$ are symmetrical around the $s_2$ and have equivalent sizes and dynamics.
% For simplicity, here we study only the dynamics of $s_3$.
% As depicted in Fig~\ref{fig: cable_dynamics}(b), at the time point when the contact is just established and there is still not deformation ($\theta = 0$), $s_3$ experiences an angular acceleration derived from $f_{push}$ that
% \begin{equation}
%    I_3 \cdot \mathbf{\ddot{\theta}} = \mathbf{L_3} \times \mathbf{f^{ff}_{push}}\textbf{,} 
% \end{equation}
% where $I_3$ is the moment of inertia of $s_3$ and $\ddot{\theta}$ is the angular acceleration.
% Once $\theta > 0$ (Fig~\ref{fig: cable_dynamics}(c)), $s_3$ will then rotate around the contact point under the moment of forces $ f^{ff}_{push}$ and $ f^{ff}_{stretch}$:
% \begin{equation}
%    I_3 \cdot \mathbf{\ddot{\theta}} = \mathbf{L_3} \times (\mathbf{f^{ff}_{push}}- \mathbf{f^{ff}_{stretch}})\textbf{.} 
% \end{equation}
% Therefore, the dynamics of $s_3$ can be described as a second-order time-invariant system. 
% If we select the magnitude of $\mathbf{f^{ff}_{push}}$ and $\mathbf{f^{ff}_{strech}}$ properly, the system will reach an equilibrium point and stops rotation and deformation.
% In this case, for a certain $\mathbf{f^{ff}_{push}}$, the larger the magnitude of the stretching force $||\mathbf{f^{ff}_{stretch}}||$ is, the sooner the system converges to the equilibrium point and the smaller the terminal deformation $\theta_T$ is when the rotation stops.
% In other words, a large $||\mathbf{f^{ff}_{stretch}}||$ enables the DLO to have a high stiffness.

In the following analysis, we ensure that we maintain a stretching force which is large enough to always keep the DLO tension. 
Therefore, $\theta$ can be considered as quasi-constant and small, and~\eqref{equ: s2_time_variant} becomes:
\begin{equation}
    ||\mathbf{f}|| = 2||\mathbf{f_s}|| \cdot sin(\theta) 
    \textbf{.}  \label{equ: fs2f}
    % \numberthis
\end{equation}

Finally, as $f_{push}^{ff}$ is designed to rise gradually from zero, at each time point before being inserted in, $s_2$ can be considered as quasi-static and the acceleration $a$ can be neglected:
\begin{equation}
    ||\mathbf{f_c}|| \approx ||\mathbf{f}||  \label{equ: f2fc}
\end{equation}



% In $X-Y$ plane, $s_2$ is under the effect of tension $f_s$ at each end as well as a contact force provided by the fixture $f_c$.
% % We assume that $s_2$ and the clip are in tight and uniform contact with each other so that the contact force can be calculated as $f_c= S_{clip} \cdot \sigma_c$, where $S_{clip}$ is the size of the contact area and $\sigma_c$ is the stress. 
% The dynamics of $s_2$ in $Y$ direction is described as
% \begin{equation} \label{equ: s2_dynamics_xy}
%     m_2 \cdot a(t)  =  2f_s \cdot sin(\theta(t)) - f_c\textbf{,}
% \end{equation}
% where $f_s \cdot sin(\theta(t))$ is the component of $f_s$ in $Y$ axis.
 
% In conclusion, with a large $f_{stretch}$, the whole DLO is rigid-like and its interaction with the clip can be analyzed based on the clip dynamics described in Section~\ref{subsec: clip_dynamics}.

% \subsection{Contact Dynamics in Anomaly}
%  Anomaly in Section~\ref{subsec: anomaly_intro} can be characteristized with the contact force provided by the clip:
%  \begin{itemize}
%      \item Missed Contact:
%  \end{itemize}

% As the object moves slowly further, the deformation as well as $f_d$ increases. 
% If the applied force is small, the acceleration may decrease to zero before the object gets inserted and the object will get stuck there. 
% In contrast, when a large force is applied, the object will pass the opening and enter the wider inner area. 
% We define the deformation which just allows the object to pass as the fixing deformation threshold $x_{open}$. 
% Once the object gets inserted, $f_a$ drops suddenly and the acceleration increases remarkably, resulting in a rapid forward movement.


% We can use time series classification to detect the anomaly and then adjust the force by trail and error.
% We look for an index that can support a real-time detection
